Technical Report: Reactive Semantic Planning in Unexplored Semantic Environments Using Deep Perceptual Feedback

This paper presents a reactive planning system that enriches the topological representation of an environment with a tightly integrated semantic representation, achieved by incorporating and exploiting advances in deep perceptual learning and probabilistic semantic reasoning. Our architecture combines object detection with semantic SLAM, affording robust, reactive logical as well as geometric planning in unexplored environments. Moreover, by incorporating a human mesh estimation algorithm, our system is capable of reacting and responding in real time to semantically labeled human motions and gestures. New formal results allow tracking of suitably non-adversarial moving targets, while maintaining the same collision avoidance guarantees. We suggest the empirical utility of the proposed control architecture with a numerical study including comparisons with a state-of-the-art dynamic replanning algorithm, and physical implementation on both a wheeled and legged platform in different settings with both geometric and semantic goals.

==> Makefile <==
#
#  Makefile for automating LaTeX related tasks and administrating a 
#  directory of numerous thesis-related files.
#
#  Prepared by Neil C. Miller
#  Modifed by Lord Simon Cuce III
#  May, 1997
#
#  Revision 2.0 5/12/97
#

INCLUDEFILES = 

	FILENAME = body
	ARCHIVE = backup
	PAPERTYPE = a4

.DEFAULT:
	@echo Sorry, that is an undefined target.

help:
	@echo
	@echo Help for make utility:
	@echo
	@echo   make	    - shows this help.
	@echo   make dvi	- executes latex one time.
	@echo   make clean      - removes all backup and output files.
	@echo   make ps	 - executes dvips one time.
	@echo   make bib	- executes bibtex one time.
	@echo   make all	- runs latex several times, bibtex and dvips.
	@echo   make backup     - creates a .tar.gz backup of all files.
	@echo
	@echo Filenames for the main document and backup archive are 
	@echo specified in the Makefile.
	@echo

%:	
	@echo "$@" | latex $(FILENAME) 

dvi:
	@echo $(INCLUDEFILES)  | latex $(FILENAME)

clean:
	@$(RM) *% *.bak *.dvi $(FILENAME).ps

realclean:
	@$(RM) *% *.bak *.dvi $(FILENAME).ps *.aux *.bbl *.blg *.ilg *.ind *.lof *.log *.lot *.lof *.toc *.loa *~

ps:
	@dvips -G0 -R0 -t$(PAPERTYPE) -o $(FILENAME).ps $(FILENAME)
goodps:
	@dvips -G0 -Ppdf -R0 -t$(PAPERTYPE) -o $(FILENAME).ps $(FILENAME)

pdf:
	dvips -G0 -Ppdf -R0 -t$(PAPERTYPE) -o tmp.ps $(FILENAME)
	ps2pdf -dCompatibilityLevel=1.4 -dMAxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=$(PAPERTYPE) tmp.ps $(FILENAME).pdf
	$(RM) -f tmp.ps

bib:
	@bibtex $(FILENAME)

# This doesn't work perfectly.  For example, the changing of a section
# name does not cause a Warning, even though its change will not be 
# reflected in the TOC until the next pass.  So, "all" should be done 
# after "realclean" before final submission.  Possibly a good use for a 
# small perl script which checks to see that the TOC is up-to-date.
all:
	echo '** Running LaTeX **'
	echo $(INCLUDEFILES) | latex $(FILENAME);
	@if ( grep "There were undefined references"        \
			$(FILENAME).log >/dev/null ); then  \
		echo '** Running BibTeX **';                \
		bibtex $(FILENAME);                         \
		echo '** Re-running LaTeX **';              \
		echo $(INCLUDEFILES) | latex $(FILENAME);  \
	fi
	@while ( grep "Rerun to get cross-references"       \
			$(FILENAME).log >/dev/null ); do    \
		echo '** Re-running LaTeX **';              \
		echo $(INCLUDEFILES) | latex $(FILENAME);  \
	done

oldall:
	@latex $(FILENAME)
	@bibtex $(FILENAME)
	@latex $(FILENAME)
	@latex $(FILENAME)

allps: all
	@dvips -G0 -Ppdf -o $(FILENAME).ps $(FILENAME)

backup:
	@$(RM) $(ARCHIVE).tar.gz
	@tar cf $(ARCHIVE).tar *
	@gzip $(ARCHIVE).tar
	@ls -l $(ARCHIVE).tar.gz


